Structured Set Matching Networks for One-Shot Part Labeling

Diagrams often depict complex phenomena and serve as a good test bed for visual and textual reasoning. However, understanding diagrams using natural image understanding approaches requires large training datasets of diagrams, which are very hard to obtain. Instead, this can be addressed as a matching problem either between labeled diagrams, images or both. This problem is very challenging since the absence of significant color and texture renders local cues ambiguous and requires global reasoning. We consider the problem of one-shot part labeling: labeling multiple parts of an object in a target image given only a single source image of that category. For this set-to-set matching problem, we introduce the Structured Set Matching Network (SSMN), a structured prediction model that incorporates convolutional neural networks. The SSMN is trained using global normalization to maximize local match scores between corresponding elements and a global consistency score among all matched elements, while also enforcing a matching constraint between the two sets. The SSMN significantly outperforms several strong baselines on three label transfer scenarios: diagram-to-diagram, evaluated on a new diagram dataset of over 200 categories; image-to-image, evaluated on a dataset built on top of the Pascal Part Dataset; and image-to-diagram, evaluated on transferring labels across these datasets.

==> 05_dataset.tex <==
% \subsection{\dataset\ Dataset}
\noindent\textbf{\dataset\ Dataset.}
We present the Diagram Part Labeling (\dataset) dataset, consisting of 4,921 images across 200 object categories. Categories span rigid objects (\eg, cars) and non-rigid objects (\eg, animals). Images are obtained from Google Image Search and parts are labelled by annotators. \dataset\ is split into train, val and test sets, with no categories overlapped. Since each pair of images within a category can be chosen as a data point, the number of data points is large (101,670 train, 21,262 val, and 20,110 test).

% Part names for each object category are obtained by asking a set of annotators to list a set of parts that are visually distinctive from one another and unique to that object category, if possible. The ten part names per category, with the most consensus are selected. For each image and part, annotators then mark points on the specified part, and the final point is chosen during a second round of annotations to choose the most representative point.

% The dataset is split into training, validation and test sets with 140, 30 and 30 categories, respectively. As per the one-shot setting, no object category is repeated between these three sets. This results in 3507, 681 and 733 images for the three categories. The number of part labeling examples is much higher however, since all pairs of images within a category can be chosen as a data point. This leads to 101,670 training, 21,262 validation, and 20,110 test examples.

\dataset\ is challenging for several reasons. First, the absence of color and dense texture cues in diagrams renders local appearance cues ambiguous. Second, having access to only point supervision~\cite{bearmanRFF16} at training time is challenging compared to having detailed segmentation annotations for parts as in previous natural image datasets (\eg, Pascal Part~\cite{chenMLFUY14}). Third, parts for several categories are located very close by, requiring very fine grained analysis of the texture-sparse diagrams (Fig.~\ref{fig:difficult_dataset}-(c)).
% Eg. \emph{beak}, \emph{comb} and \emph{wattle} parts in the \emph{chicken} category are all very close by (Figure~\ref{fig:difficult_dataset}-(c)). 
Fourth, the appearances and locations of parts are generally not coherent across samples within a category. Finally, the one-shot setting renders this even more challenging.

% \begin{figure}[t]
% 	\centering
%     \includegraphics[width=0.20\linewidth]{figures/data_hard_chicken_10part.pdf}~
%     \includegraphics[width=0.38\linewidth]{figures/data_hard_airplane_10part.pdf}
%     \includegraphics[width=0.38\linewidth]{figures/data_hard_hairdryer_10part.pdf}\\
%     {\small \hspace{-1em}(a)\hspace{7.5em}(b)\hspace{9em}(c)}
%     \caption{Challenging examples in \dataset. (a) Spatially close parts (b) Missing in the diagram (c) Occluded by other parts}
%     \vspace{-1em}
%     \label{fig:dataset_hard}
% \end{figure}


% For the one-shot setting, object categories do not overlap between the training, validation and testing sets. However, some common part names happen to overlap between these sets, \eg, animal categories typically have parts such as \emph{leg} and \emph{eye}. 51\% of the part names in the validation set and 54\% in the test set appear in the training set. Our analysis (Section~\ref{sec:parts_help}) shows that in spite of this overlap, learning part appearances provides no benefit to the model. The \dataset\ dataset will be publicly released.


% \choi{(TODO: showing overlap of super categories of categories.)}


% \subsection{\datasettwo\ Dataset}
\vspace{.5em}
\noindent\textbf{\datasettwo\ (PPM) Dataset.}
To evaluate SSMN on labeling parts in natural images, we use images from the Pascal Part dataset~\cite{chenMLFUY14} with more than 10 parts and convert part segments to point annotations using the centers of mass. We called it Pascal Part Matching (PPM), which consists of 74,660 train and 18,120 test pairs in 8 categories with 10 parts.



\vspace{.5em}
\noindent\textbf{Cross-DiPART-PPM Dataset.}
For cross domain matching experiments, we find all overlapping categories and part names between \dataset\ and \datasettwo\ to make Cross-DiPART-PPM. It consists of 5 categories with 4 parts and 22,969 image-to-diagram pairs (18,489 train and 4,480 test).
\emph{All datasets will be publicly released. Supplementary material contains more details.}

==> 06_exp.tex <==

\begin{figure*}[t]
    % \includegraphics[width=0.33\linewidth]{figures/quali_shrimp10.pdf}
    % \includegraphics[width=0.33\linewidth]{figures/quali_cicada10.pdf}
    % \includegraphics[width=0.33\linewidth]{figures/quali_mosquito10.pdf}
    % \includegraphics[width=0.33\linewidth]{figures/quali_shrimp10.pdf}
    % \includegraphics[width=0.33\linewidth]{figures/quali_ppm10_cat.pdf}
    % \includegraphics[width=0.33\linewidth]{figures/quali_cross_horse.pdf}
    \includegraphics[width=0.33\linewidth]{figures/quali_dipart10_shrimp2a.pdf}   
    \includegraphics[width=0.33\linewidth]{figures/quali_ppm10_cat2a.pdf}
    \includegraphics[width=0.33\linewidth]{figures/quali_cross_horse2a.pdf}    
    \caption{Qualitative results from our SSMN model. In each pair of images, the labeled source images is on the left and the target is on the right. A green box indicates a correct match and a red box indicates an incorrect match.}
    \vspace{-1em}
    \label{fig:quali_result}
\end{figure*}

\begin{figure*}
    \centering
    % \includegraphics[width=0.75\linewidth]{figures/iteration_steps_2row.pdf}
    % \includegraphics[width=0.95\linewidth]{figures/iteration_steps_single_row.pdf}
    \includegraphics[width=0.95\linewidth]{figures/iteration_steps_single_row2.pdf}
    \caption{Visualization of expected part locations during the search by the structural consistency factor ($f_{sc})$.
    The example has both the varying pose and a non-trivial transformation of source to target part locations.
    The matched parts of each diagram are represented by the color-coded points.
    Each color-coded heatmap shows the score assigned by the structural factor to every location in the diagram for the unmatched part with the same color.
    % Top: an easy example of left-right inversion. 
    % Bottom: a challenging example where both the pose is varied and the part annotations are in different locations. 
    For visual clarity, we display 5 of the 10 parts.
    }
    \vspace{-1em}
    \label{fig:structural_factor}
\end{figure*}

\noindent\textbf{Set-up.}
Training neural networks with global normalization typically requires pre-training with log-likelihood to obtain good results \cite{Andor2016,Wiseman2016SequencetoSequenceLA}. In training the SSMN, we pretrained it using the appearance matching network (AMN) surrogate objective (Sec~\ref{sec:training}), then fixed the weights of the convolutional layers while retraining the remainder of the network with 1 epoch of LaSO with a beam size parameter of 5 in most experiments unless mentioned (as described in Sec~\ref{sec:training}). We found that additional training epochs did not improve accuracy, presumably because pre-training brought the parameters close to a good solution. At test time, we ran the SSMN with a beam size of 100 in all experiments, except the ones that measured accuracy at different beam sizes. We chose this number based on experiments on the validation set which found that accuracy plateaued beyond 100.

The \emph{encoder network} uses two convolutional layers (64 filters of $3 \times 3$ and 96 filters of $3 \times 3$), each followed by $2 \times 2$ max pooling with stride of 2. This is followed by two fully connected layers, with 128 and 64 hidden units respectively. The \emph{context network} is a single layer bidirectional LSTM with 50 hidden units. We train the network using SGD with momentum and decay and $10^{-4}$ initial learning rate.

Note that the datasets we used in all the evaluations have no categories overlaps in train and test splits. It is a challenging set-up that matching the appearances of source and target that are never seen in training phase.

\begin{table}[t]
    \centering
    \begin{tabular}{lcc} 
        \toprule
        Methods $\backslash$ Dataset & \dataset\ & PPM \\
        \hline
%        {\rowcolor[gray]{0.92} \footnotesize \textsf{Independent Matching Methods}} & & \\ 
%        \hline
        Random                      & 10.0\% & 10.0\%\\
        Nearest Neighbor (RGB)      & 29.4\% & 11.1\%\\
        Affine Transform            & 32.1\% & 26.9\%\\
        UCN~\cite{Choy2016UniversalCN}         
                                    & 38.9\% & 20.2\%\\
        % SCNet-AG+~\cite{hanRHWCSP17}
        %                             & ----\% & ----\%\\
        Matching Network (MN)~\cite{vinyalsBLKW16}    
                                    & 41.3\% & 40.2\%\\
        $^\llcorner$ MN-ContextLSTM      
                                    & 38.4\% & 40.5\%\\
        $^\llcorner$ MN+Hungarian        
                                    & 45.6\% & 42.7\%\\ % MN+Hungarian
        \hline
        Appearance Matching Network+NN   
                                    & 35.7\% & 42.3\%\\ % +matching is 48.9
        SSMN-GlobalConsist
                                    & 44.7\% & 40.6\%\\
        \textbf{SSMN (Ours)}
                                    % & \textbf{54.2}\% & \textbf{44.4}\%\\
                                    & \textbf{58.1}\% & \textbf{46.6}\%\\
        \bottomrule
    \end{tabular}
    \caption{Accuracies of SSMN and other methods on both datasets.}
    \vspace{-1em}
    \label{tab:results_10part}
\end{table}


\vspace{.5em}
\noindent\textbf{Baselines.}
We compare SSMN to the following baselines.

\noindent \textbf{Nearest Neighbor (RGB)} computes matches using local appearance cues only by comparing raw image patches centered on the part's point using a euclidean metric.

\noindent \textbf{Affine transform} baseline selects the matching of points that minimizes the error of a least-squares fit of the target part locations given the source part locations. This is not scalable to compute exactly, as it requires running a least-squares fit for every matching (3.7 million for 10 part matchings). We ran this approximately using beam search with width equal to 100.

\noindent \textbf{Matching Network (MN)}~\cite{vinyalsBLKW16} independently predicts a source point for each target point. This network runs the appearance matching network described in Section \ref{sec:appearance_similarity}, \ie. the encoder network with bidirectional LSTMs, to score each source given a target. The network is trained by feeding these scores into a $K$-way softmax then maximizing log-likelihood. A limitation of MN is that it does not enforce a 1:1 matching, hence may yield an invalid solution.

\noindent \textbf{MN + Hungarian} solves this problem by finding the maximum weighted matching given the matching network's scores. In contrast to the SSMN, this baseline uses the Hungarian algorithm as a post-processing step and is not aware of the matching constraint during training.

\noindent \textbf{MN - Context LSTM} removes the context LSTM and is designed to evaluate the effectiveness of using a sequential context mechanism on a set of elements.

\noindent \textbf{Appearance Matching Network + NN} computes nearest neighbor matches using only appearance cues by the Appearance Matching network. Source and target points are fed into the encoders and matched using cosine similarity.

\noindent \textbf{Universal Correspondence Network (UCN)}~\cite{Choy2016UniversalCN} originates from the the semantic correspondence (SC) matching literature. 
Minimal post processing was required to adapt it to our task and compute an accuracy metric comparable to the SSMN and other baselines. 
%We post-process the PCK measure to labeling accuracy by finding nearest annotated point from the matched correspondence.
Best results were obtained when fine tuning their pre-trained network on our datasets.

%\choi{For the relevance to the semantic correspondence (SC) matching literature, we also compare the performance of the SSMN to the Universal Correspondence Network (UCN)~\cite{Choy2016UniversalCN} on DiPART dataset. Unlike the previous work in the SC literature reporting the accuracy by PCK, our labeling performance is on exact matching. Thus, we compute the nearest key point among the candidate locations in the target image from the matched correspondence in the target image. By UCN on \dataset\, we obtain 40.8\% accuracy, which is slightly better than the performance of our appearance matching network (AMN). In UCN, we use spatial transformer network and fine-tune the GoogLeNet (or Inception)~\cite{szegedyLJSRAEVR15} trained on ImageNet 2014 challenge dataset while our model is trained from the scratch only on the \dataset\ dataset.

Very recently, Han \etal~\cite{hanRHWCSP17} proposed the SCNet for learning a geometrically plausible model for semantic
correspondence. We worked closely with the authors to adapt their SCNet code for our task and datasets, but were unable to obtain satisfactory results (\dataset: 11.1\%, \datasettwo: 11.2\%). 

%But training SCNet on both of our dataset is not trivial as we do not use part segmentation in PPM and lack of texture in \dataset\ and its performance is not satisfactory.\footnote{We work closely with the authors of SCNet to train the network.}
% The main gain of the SCNet comes from the robustness large deformation of the regions but our dataset only provides point annotations thus training SCNet is not trivial and its performance is not satisfactory.\footnote{We work closely with the authors of SCNet to train the network.}

% The final baseline, Affine Transform, is an unsupervised approach that selects the matching of the points that minimizes the error of a least-squares fit of the target part locations given the source part locations. This method can be viewed as making a simple global consistency assumption -- that the transformation from source to target is affine -- and finding the best matching under this assumption. (Note that this baseline is not scalable, as it requires running a least-squares fit for every matching (3.7M for 10 part matchings).)

Table \ref{tab:results_10part} compares the accuracy of SSMN with the above baselines on the test sets for the DiPART and PPM datasets. The nearest neighbor baselines (both RGB and Appearance Matching Network) perform poorly, since they only use appearance cues with no contextual information and no matching constraint. The MN-ContextLSTM model performs better that the nearest neighbor model. The MN model easily outperforms MN-ContextLSTM, which clearly demonstrates that using sequential context, even in a set environment yields good results, consistent with the findings in~\cite{vinyalsBLKW16}. Enforcing a 1:1 matching constraint via the Hungarian algorithm further improves this model. SSMN also outperforms UCN on both datasets. The SSMN outperforms other baselines because of its ability to model global consistency among the source and target sets. Training with global normalization is crucial to obtaining this improvement: if we instead train SSMN with local normalization, accuracy drops significantly (SSMN-GlobalConsist). 
 

\vspace{.5em}
\noindent\textbf{Effect of beam size.}
Fig.~\ref{fig:beam_size} shows the test accuracies as a function of inference beam size. SSMN outperforms baselines even for beam sizes as low as 10, and saturates beyond 100. Note that even a beam size of 100 represents a tiny fraction ($0.0027\%$) of the search space of matchings ($10!$).

% 
% \begin{table}[h]
%    \centering
%    \begin{tabular}{l|r} 
%        \toprule
%        Beam Size & SSMN Accuracy \\
%        5 &  62.4 \\
%        10 & 65.7 \\
%        20 & 67.1 \\
%        30 & 67.4 \\
%        40 & 67.4 \\
%        50 & 67.5 \\
%        \hline
%    \end{tabular}
%    \caption{Effect of beam size on SSMN accuracy.}
%    \label{tab:ssmn_beamsize}
% \end{table}

\begin{figure}[h]
	\centering
    \includegraphics[width=0.95\linewidth]{figures/beamsize_plot.pdf}
    \caption{Accuracy as a function of inference beam size.}
    \vspace{-1em}
    \label{fig:beam_size}
\end{figure}


\vspace{.5em}
\noindent\textbf{Distance Transform (DT).}
We propose using DT images as inputs to our encoder networks, as opposed to the original diagrams. We compared the two approaches using just the appearance matching network, in order to isolate appearance cues from structural cues. Using DT images provides an accuracy of $38.4\%$ where as the original image produces $33.5\%$, a noticeable improvement. An interesting observation was that when we swept the space of filter sizes to find the best performing one for each configuration, the best filters for the original image were $15\times15$ as reported in~\cite{Yu2016SketchaNetAD} but the best filters for the DT image was $3\times3$, which is consistent with CNN architectures built for natural images.

%\begin{table}[h]
%    \centering
%    \begin{tabular}{ccc}
%        \toprule
%                        & Original Image    & DT-image \\
%        \hline
%        Test Accuracy   & 33.5\%            & 38.4\% \\
%        \bottomrule
%    \end{tabular}
%    \caption{Labeling accuracies of Appearance Matching Network (AMN) followed by the MN-ContextLSTM model with different input image type in \dataset\ test split. DT-image denotes Distance-transformed image.}
%    \label{tab:dist-transform}
%\end{table}

\vspace{.5em}
\noindent\textbf{Does General Part Appearance Help?}
\label{sec:parts_help}
51\% of part names in the validation and 54\% in the test set appear in the training set of \dataset. Hence one might expect the part appearance factor ($f_p$) in SSMN to help significantly. An ablation study found that removing it caused very little drop in validation accuracy (within 0.1\%). This shows that, even though part names overlap significantly, part appearance cues do not always transfer between categories; \eg, a \emph{head} of an elephant and a giraffe look significantly different.

%\note{todo}: Other possible baselines: pointer network?
%\choi{class-wise analysis to say something about dataset itself and the algorithm's pros and cons.}

%\subsection{SSMN Ablations}
%Table \ref{tab:ssmn_ablations} shows the results of an ablation experiment to measure the contribution of each component of SSMN to its overall accuracy. The first three variants are versions of SSMN trained without one of its factors. Comparing the accuracies of these variants demonstrates that structural consistency is largely responsible for SSMN's improvement over MatchingNet -- removing this factor reduces accuracy to 55.3, which is similar to that of the MN+Hungarian baseline. Note that we do not expect these numbers to be identical, as SSMN uses approximate inference and has a different training objective.The final variant trains SSMN with local normalization and loglikelihood, to measure the importance of global normalization. This model predicts a matching in a sequential fashion, where at each time step it is given a target point and it produces a probability distribution over the unmatched source points. This model is trained to maximize the loglikelihood of the correct source point at each time step, i.e., it is trained analogously to a sequence RNN. We find that removing global normalization dramatically reduces the accuracy of SSMN because the structural consistency factor is no longer effective. Figure \ref{fig:structural_factor} visualizes the information learned by the structural consistency factor when SSMN is trained with global normalization.

%\begin{table}[h]
%    \centering
%    \begin{tabular}{lr} 
%        \toprule
%        MatchingNet \note{todo: name} & 68.7 \\
%        ~ $+$ part appearance $(f_p)$ & 68.5 \\
%        ~ $+$ global consistency $(f_{gc})$ & 73.8 \\
%        \bottomrule
%    \end{tabular}
%    
%    \begin{tabular}{lr} 
%        \toprule
%        SSMN & 67.1 \\
%        \hline
%          w/o part appearance $(f_p)$ & 66.0 \\
%          w/o appearance matching $(f_a)$ & 65.6 \\
%          w/o structural consistency $(f_s)$ & 55.3 \\ 
%          w/o global normalization & 47.0 \\
%          \bottomrule
%    \end{tabular}
%    \caption{Adding factors to MatchingNet to reach SSMN. The two global consistency factors yield
%    the highest accuracy improvements.}
%    \label{tab:ssmn_ablations}
%\end{table}

\vspace{.5em}
\noindent\textbf{Qualitative Analysis.}
Figure~\ref{fig:quali_result} shows qualitative examples and Figure~\ref{fig:structural_factor} visualizes SSMN's search procedure. More results can be found in the supplementary material.

%We show examples of qualitative results in Fig.~\ref{fig:quali_result}.
%Although the visual appearance of the parts are distinctive and their spatial locations are not consistent, our SSMN model finds the parts by learning the discriminative appearance with the global constraints.
%In the right most example, as wing in the 
%
%We also show the expected part locations as predicted at each optimization search procedure by the structural consistency factor ($f_{sc}$) in Fig.\ref{fig:structural_factor}.
%The matched parts of each diagram are represented by the color-coded points.
%The next three diagrams show partial matchings of target parts produced as SSMN inference proceeds along with a heatmap of the scores assigned by the structural factor to every position in the diagram for the remaining parts.
%An easy example (first row of the figure) of left-right inversion. The positions of the parts expected in the first step are essentially correct.
%A challenging case (second row) where both the pose is varied and the part annotations are in different locations. The factor's predictions are reasonable, but unfortunately not helpful.
%Note that, at inference time, it is only necessary to evaluate the factor at the marked part locations, not at every point in the diagram.

% \begin{figure*}[t]
% 	\hspace{-1em}
% 	\begin{tabular}{cc}
%         \includegraphics[width=0.49\linewidth]{figures/quali_shrimp.pdf}&
%         \includegraphics[width=0.49\linewidth]{figures/quali_minivan.pdf}\\
%         \includegraphics[width=0.49\linewidth]{figures/quali_turtle.pdf}&
%         \includegraphics[width=0.49\linewidth]{figures/quali_mosquito.pdf}
%     \end{tabular}
%     \caption{Qualitative results by our SSMN model. In each example, left image is the source with label, right image is the target. Green box indicates correct match, red box indicates wrong match.}
%     \label{fig:difficult_dataset}
% \end{figure*}



% The DiPART data set consists of 5000 diagrams, each of which is annotated with 5 parts, of objects from 200 categories. These categories are split into a 150 / 25 / 25 train / validation / test split. Therefore, at test time, every diagram belongs to a category unseen during training. Although these categories are unseen during training, some part names are shared. We calculated that 51\% of the part names in the validation set and 54\% of those in the test set appear in the training set. This moderate overlap suggests that learning part appearances may be helpful in some cases, but insufficient in general.

\vspace{.5em}
\noindent\textbf{Matching Variable Numbers of Parts.}
\dataset\ and PPM are setup to contain a fixed number of parts across images and a complete 1:1 matching between source and target sets. However, SSMN makes no such strict assumptions and can also be used in a relaxed setups. We modified \dataset\ to contain 9 parts in the source and 8 parts in the target image. 7 of these have a 1:1 matching and 1 part in each set has no correspondence in the counterpart. Table~\ref{tab:varypart} compares SSMN to the strongest baseline (MN+Hungarian). As 1:1 matching is not guaranteed, the Hungarian algorithm only marginally improves accuracy over MN while SSMN still provides large improvements.
\begin{table}[h]
    \centering
    \begin{tabular}{cccc}
        \toprule
                        & MN        & MN+Hungarian  & SSMN       \\
        \hline
        Test Accuracy   & 31.1\%    & 31.5\%        & 38.2\% \\
        \bottomrule
    \end{tabular}
    \caption{Accuracies in DiPART with varying part setup.}
    \vspace{-1em}
    \label{tab:varypart}
\end{table}


\vspace{.5em}
\noindent\textbf{Cross Domain Matching.}
We evaluate cross domain matching on Cross-DiPART-PPM. This is the most challenging among the three setups. By using different \emph{encoder network} architecture for source and target, we demonstrate that SSMN is able to transfer labels across domains (images-to-diagrams) reasonably well. Since global geometric consistencies are preserved regardless of visual signatures, the SSMN outperforms the strongest baseline (Table~\ref{tab:crossdomain}). In this setup, the part classification term ($f_p$, Sec.~\ref{sec:part_appearance}) drops performance since the part classifiers do not generalize across domains. Thus, SSMN without $f_p$ (SSMN-$f_p$) provides further improvements.

\begin{table}[h]
    \centering
    \resizebox{8.1cm}{!}{
    % \begin{tabular}{cccccc}
    %     \toprule
    %                     & MN-C  & MN        & MN+Hungarian  & SSMN & SSMN-RelAppr\\
    %     \hline
    %     Test Accuracy   & 32.4  & 28.0\%    & 26.4\%        & 30.8 & 33.1\% \\
    %     \bottomrule
    % \end{tabular}
    \begin{tabular}{cccccc}
        \toprule
                        & Random & MN        & MN+Hungarian  & SSMN & SSMN-$f_p$\\
        \hline
        Test Accuracy   & 25\%   & 28.0\%    & 26.4\%        & 30.8\% & 33.1\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Cross domain accuracies (Cross-DiPART-PPM data)}
    \vspace{-1em}
    \label{tab:crossdomain}
\end{table}

